DeepStream: Bandwidth Efficient Multi-Camera Video Streaming for Deep Learning Analytics

Deep learning video analytic systems process live video feeds from multiple cameras with computer vision models deployed on edge or cloud. To optimize utility for these systems, which usually corresponds to query accuracy, efficient bandwidth management for the cameras competing for the fluctuating network resources is crucial. We propose DeepStream, a bandwidth efficient multi-camera video streaming system for deep learning video analytics. DeepStream addresses the challenge of limited and fluctuating bandwidth resources by offering several tailored solutions. We design a novel Regions of Interest detection (ROIDet) algorithm which can run in real time on resource constraint devices, such as Raspberry Pis, to remove spatial redundancy in video frames and reduce the amount of data to be transmitted. We also propose a content-aware bandwidth optimization framework and an Elastic Transmission Mechanism that exploits correlations among video contents. We implement DeepStream on Raspberry Pis and a desktop computer. Evaluations on real-world datasets show that DeepStream's ROIDet algorithm saves up to 54\% bandwidth with less than 1\% accuracy drop. Additionally,DeepStream improves utility by up to 23\% compared to baselines under the same bandwidth conditions.

==> SpaTem.tex <==
\section{Adaptation to Spatial Temporal Correlations}
\label{sec:spatem}

Since \name{} targets network scheduling for a fleet of cameras deployed within the same network, the cameras are spatially co-located and therefore spatial temporal correlations exist among the cameras \cite{jain2020spatula}. The number and size of cars these cameras capture at a certain time slot are correlated. As we perform Regions of Interest based frame cropping in Section~\ref{sec:cam}, the areas of Regions of Interest are also correlated across the cameras, as shown in Figure~\ref{fig:roi_area}. When there are large areas of Regions of Interest to transmit to the edge server, we need higher bitrate videos so that we can maintain a high compression quality and thereafter high detection accuracy. When the Regions of Interest are small, high bandwidth allocation is not needed. To demonstrate this, we encode profiling video feeds from all cameras into the same bitrate ($100kbps$) and show the relationship between total area of ROIs and the sum of detection accuracy across all cameras in Figure~\ref{fig:roi_acc}. Moreover, network bandwidth conditions vary over time. When more bandwidth is needed to encode larger Regions of Interest, this requirement may not be satisfied by the current network conditions. 
Based on these observations, we propose a novel Elastic Transmission Mechanism for \name{}. 

 \begin{figure}
  	\centering
  	\includegraphics[width=1\linewidth]{figures/roi.png}
	\caption{The area of ROIs of each camera on each video segment of $1s$ from the profiling dataset.}
	\label{fig:roi_area}
\end{figure}
 \begin{figure}
  	\centering
  	\includegraphics[width=1\linewidth]{figures/acc_roi.png}
	\caption{The relationship between total ROIs area across all cameras and segment utility (we assign the same weights to all cameras here). All videos are encoded into $100kbps$ segments.}
	\label{fig:roi_acc}
\end{figure}



The high-level idea of the Elastic Transmission Mechanism is that, when the cameras demand high bandwidth as a result of large Regions of Interest areas and the network conditions do not permit the demanded bandwidth, the Elastic Transmission Mechanism borrows transmission time from future time slots to help with video transmission of the current time slot. Note that this mechanism is different from simply adapting bandwidth allocation to network conditions, since the Elastic Transmission action is driven by video contents (ROIs area).  This mechanism works as follows.

\textbf{Thresholds Selection.}
 \name{} performs an analysis to obtain two thresholds --- a threshold on the total area of Regions of Interest among all cameras to decide whether more transmission time is needed beyond the current time slot, and a threshold on current bandwidth condition to decide whether it's sufficient to encode video segments with large Regions of Interest. If the total area of Regions of Interest is larger than its threshold and the current network bandwidth is smaller than its threshold, \name{} borrows transmission time from future time slots.

To obtain the threshold on area of Regions of Interest, \name{} keeps a moving average of the area of Regions of Interest $\hat{a}^{(t)}=\alpha a^{(t)}+(1-\alpha)\hat{a}^{(t-1)}$ where $a$ represents the total area of Regions of Interest across all cameras, and the standard deviation $\sigma_a$ of Regions of Interest area. The threshold can therefore be expressed as 
    $\tau_a = \hat{a}^{(t)} + \lambda_a \sigma_a$, 
where $\lambda_a$ is a parameter controlling the aggressiveness of elastic transmission.

In order to obtain the threshold on bandwidth conditions, \name{} first selects the configuration that achieves the highest detection accuracy corresponding to each bitrate option, as is expressed on Line 2 of Algorithm~\ref{al:bwalloc}. For each bitrate option $b$ and for each camera $i$, \name{} calculates the average and standard deviation of the differences in accuracy between encoding in bitrate $b_i$ and encoding in highest possible bitrate $b_M$ over all video segments in the training set. When the average and standard deviation of the accuracy differences is below preset values\footnote{The preset value for average and standard deviation in differences are selected empirically.}, \name{} selects the sum of corresponding bitrates $\tau_{wl}=\Sigma_i b_i$ as a threshold of demanding more transmission time. When the average and standard deviation of the accuracy differences is above preset values, \name{} selects the corresponding bitrate sum as a threshold $\tau_{wh}$ of being able to give back transmission time.

\textbf{Transmission Adjustment.}
When the current area of Regions of Interest is larger than its threshold and the current bandwidth is smaller than its threshold: $a^{(t)}>\tau_a$ and $W^{(t)}<\tau_{wl}$, \name{} borrows transmission resources from future time slots. The amount of resources borrowed is expressed in the amount of data that can be transmitted given extra transmission time from future: $D=\lambda_{wl}(\tau_{wl}-W^{(t)})T$. We define a concept Elasticity represented by $E$, representing the maximum amount of data that \name{} can borrow without giving back. Naturally, $D$ shouldn't be larger than $E$. On the other hand, when the current bandwidth $W^{(t)}>\tau_{wh}$, \name{} starts to replenish $E$ with the filled amount to be $D=\lambda_{wl}(\tau_{wh}-W^{(t)})T$, which is a negative number. $\lambda_{wl}$ and $\lambda_{wh}$ control how aggressive \name{} borrows and gives back transmission resources. When we decide the amount of data to borrow or give back, we modify the second constraint in Equation~\ref{equ:opt} to be $\Sigma_i b_i^{(t)} T\leq W^{(t)}T+D$.

